Observations of the Onset of Complex Organic Molecule Formation in Interstellar Ices

Isolated dense molecular cores are investigated to study the onset of complex organic molecule formation in interstellar ice. Sampling three cores with ongoing formation of low-mass stars (B59, B335, and L483) and one starless core (L694-2) we sample lines of sight to nine background stars and five young stellar objects (YSOs; A_K ~0.5 - 4.7). Spectra of these stars from 2-5 $\mu$m with NASA's Infrared Telescope Facility (IRTF) simultaneously display signatures from the cores of H$_2$O (3.0 $\mu$m), CH$_3$OH (C-H stretching mode, 3.53 $\mu$m) and CO (4.67 $\mu$m) ices. The CO ice is traced by nine stars in which five show a long wavelength wing due to a mixture of CO with polar ice (CO$_r$), presumably CH$_3$OH. Two of these sight lines also show independent detections of CH$_3$OH. For these we find the ratio of the CH$_3$OH:CO$_r$ is 0.55$\pm$0.06 and 0.73$\pm$0.07 from L483 and L694-2, respectively. The detections of both CO and CH$_3$OH for the first time through lines of sight toward background stars observationally constrains the conversion of CO into CH$_3$OH ice. Along the lines of sight most of the CO exists in the gas phase and $\leq$15% of the CO is frozen out. However, CH$_3$OH ice is abundant with respect to CO (~50%) and exists mainly as a CH$_3$OH-rich CO ice layer. Only a small fraction of the lines of sight contains CH$_3$OH ice, presumably that with the highest density. The high conversion of CO to CH$_3$OH can explain the abundances of CH$_3$OH ice found in later stage Class 1 low mass YSO envelopes (CH$_3$OH:CO$_r$ ~ 0.5-0.6). For high mass YSOs and one Class 0 YSO this ratio varies significantly implying local variations can affect the ice formation. The large CH$_3$OH ice abundance indicates that the formation of complex organic molecules is likely during the pre-stellar phase in cold environments without higher energy particle interactions (e.g. cosmic rays).

==> Deleted_Text.tex <==
\section{Results}\label{sec:Results}

From our 14 targets we detect 10 sources with H$_2$O ice, five of which also have CO ice, and one that has CH$_3$OH ice above a 3$\sigma$ level. The absorption strengths are determined and converted to column densities and abundances using intrinsic integrated band strengths as done in Boogert et al. (2011) and  Boogert et al. (2013).  The ice absorption features are shown for each spectrum in Figure \ref{fig:spectra_tau}.  Where the ices are detected we can determine the ratios of the abundances of the different ices (Table 3).

\begin{figure}[h!tb]
\centering
\includegraphics[scale=0.65]{Images/spectra_tau.pdf}
\caption{All Spectra and Optical Depth plots}
\label{fig:spectra_tau}
\end{figure}

\subsection{Ices at Different A$_V$}

Our sample allows us to measure the column density of ice for a variety of extinction levels.  At lower levels of extinction and warmer temperatures \hto will freeze out and only at higher densities where the temperature decreases will we detect CO and \choh ices (Boogert, Gerakines, and Whittet 2015).  In Figure \ref{fig:ColDensity_AV} we show this relation for our targets including calculated upper limits as described in section \ref{sec:Upper Limts}.  This is compared to other data in the literature and we find a good agreement with the relation.  We also extend the relation of CO out to higher levels of extinction than previously measured and find that the relationship continues to show a linear relationship.


\begin{figure}[h!tb]
\centering
\includegraphics[scale=0.65]{Images/ColDensity_Av.png}
\caption{The column density as a function of A$_V$ for lines of sight through dense cores.  This figure from Boogert, Gerakines, and Whittet (2015) displays data taken from  Chiar et al. (1995), Whittet et al. (2007), Boogert et al. (2011), Chiar et al. (2011), Whittet et al. (2013) and Boogert et al. (2013).  Overplotted is data from this work in colored circles outlined in black (yellow for \hto, green for CO, and blue for \choh. }
\label{fig:ColDensity_AV}
\end{figure}


\subsection{\choh Detection}\label{sec:choh detection}

As mentioned previously, we require the detection of \choh ice to have a strong absorption band at 3.53 $\mu$m and we only have a firm detection \choh in one source: 2MASS J19410754+1056277 .  The source is not our highest extincted object (A$_V \sim$23) and it is not the most evolved core (L694-2, a collapsing core). This agrees with Boogert et al. 2011 that the abundance varies depending on the environment and conditions of the cores.  Some of the other sources in our sample were also limited by signal to noise and for those sources we determine the upper limits.

\begin{figure}[h!tb]
\centering
\includegraphics[trim={0 13cm 0 0},clip, scale=0.55]{Images/CH3OH_tau.pdf}
\caption{The optical depth for the C-H stretching mode of the \choh feature for 2MASS J19410754+1056277. A Gaussian fit to the feature is shown in red using methods described in Section \ref{sec:choh detection}}
\label{fig:CH3OH}
\end{figure}

%trim={0,2cm,0,0}


\begin{figure}[h!tb]
\centering
\includegraphics[trim={0 13cm 0 0},clip,scale=0.55]{Images/CO_Elias16_Compare.pdf}
\caption{The optical depth of CO for 2MASS J19410754+1056277 (black) and in Elias 16 (scaled to match, in red).}
\label{fig:COElias}
\end{figure}


From intro:

The discovery of exoplanets has shown that there must be a relatively common process to build up grains to form planetary bodies.  In dense molecular clouds the freeze-out of gases onto cold dust grains build up ice mantles that could lead to the growth needed to build larger bodies.  These molecules (H$_2$O, CO, CO$_2$, \choh, NH$_3$, etc.) are essential in understanding the early composition of our own solar system, however the prevalence of these molecules and the conditions promoting or inhibiting their formation (e.g., density, time scales, stellar feedback) are currently not well observationally constrained.

While there are prolific studies of the distribution of H$_2$O, CO$_2$, and CO gas features in molecular clouds, previous studies on the ice features have mainly focused on low mass YSOs at a more evolved stage in prestellar evolution.  Very few studies have actually probed background stars of quiescent or collapsing molecular clouds for all three ices \citep{Whittet1998, Gibb2004, Noble2013}.  Some observations have studied either \hto (3.0 $\mu$m), \choh (3.53 $\mu$m), or CO (4.67 $\mu$m) ices from the ground (CO$_2$ has too much telluric absorption) but not usually simultaneously for the same stars (e.g. \cite{Whittet1985, Whittet1989, Eiroa1989, Boogert2011}).

\subsection{CO at High A$_V$}

We see from Figure \ref{fig:Ak_tau} that CO still exists for background stars even at high levels of extinction.  The hydrogenation of CO to H$_2$CO and \choh would potentially deplete reservoirs of CO and the column density of CO at denser parts of the core would not increase as steadily as the lower column densities.  We do see that the slope of the fit to the data is more shallow than previously derived by \citet{Chiar1995}, indicating we may see a small decrease in CO at higher levels of extinction, but we have too few sources at high levels of A$_K$ to conclusively show any turnoff where CO appears to be depleted due to an increase in other ice formation.  Also, the source 2MASS J19410754+1056277 shows an excess of CO ice compared to the derived trend even though we have an independent detection of \choh ice. 

 %Both 2MASS J18172690-0438406 and 2MASS J19410754+1056277 have a similar brightness in the M band and were observed for similar durations but the higher S/N for 2MASS J19410754+1056277 comes from being observed near zenith. 
 
 %However we find that the amount of \choh is underestimated in our measurements by almost a factor of 2$\sigma$ based on the errors in \citet{Boogert2011}.  This could be due to noise in the center of the feature in our data causing a more shallow Gaussian fit to the feature or it could be the difference in the baseline chosen for the feature \textcolor{red}{Still need to compare with the data from Adwin}.  Ignoring the noise from the center of the feature, the fit from \citet{Boogert2011} does fit the wings as seen in Figure \ref{fig:CH3OH_ice} thus the measurements appear to be in agreement.  Both 2MASS J18172690-0438406 and 2MASS J19410754+1056277 have a similar brightness in the M band and were observed for similar durations but the higher S/N for 2MASS J19410754+1056277 comes from being observed near zenith. 
 
 %For the first time we have simultaneously measured the CO and \choh ice features for background targets to observationally understand the early stage that may assist in the formation of COMs.  As shown in Section \ref{sec:COice} the CO feature can be broken into individual components.  The narrow central feature of the CO ice band is attributed to CO embedded in a species with a low (apolar) dipole moment and the red component comes from a higher (polar) dipole moment \citep{Sandford1988} now believed to be a mixture of CO with CH$_3$OH ice \citep{Cuppen2011}.  Five of our targets display this red wing feature above a 3$\sigma$ confidence level.  Two of these sources also have clear \choh ice features at 3.53 $\mu$m (2MASS J18172690-0438406 in L483 and 2MASS J19410754+1056277 in L694-2).  For these cases it is reasonable to expect the polar CO wing to be caused by a mixture of CO with \choh ice.
 
 In Table \ref{tab:col density} we report the ratio of \choh:CO$_{\text{polar}}$.  For 2MASS J18172690-0438406 we find \choh:CO$_{\text{polar}}=0.46 \pm 0.06$ and for 2MASS J19410754+1056277 \choh:CO$_{\text{polar}}=0.73 \pm 0.07$.  This ratio is similar to that of low-mass YSO L1489 (\choh:CO$_{\text{polar}}=0.40)$ but not as high as the massive YSO ratio (\choh/CO$_{\text{polar}}=1.70$) \citep{Boogert2008, Pontoppidan2008}.  The first source samples an isolated core with a Class 0 low-mass YSO (L483) while the second samples a starless collapsing core (L694-2) which confirms that the process to form \choh abundantly from CO is possible early on. We also demonstrate it is possible to have a larger fraction of \choh ice than some low-mass YSOs.
 
 %(CO Ice freeze out) This cannot be explained by the conversion of CO to CH$_3$OH and thus our columns are mostly dominated by the lower extinction regions of the core where CO still remains in the gas phase.  The ice observations seem to only trace a small fraction of the overall core volume wherein much of the CO is frozen out and \choh is formed.  We note that the target 2MASS J19410754+1056277 has the highest CO$_{\text{ice}}$:CO$_{\text{total}}$ ratio and also the highest \choh abundance.  Without more sources we cannot identify this as a correlation as the local environment such as the density may still have an impact on the ice formation. 
 
 the first one also has the highest extinction in our sample (where we use extinction value based on the A$_V$ reported in Table \ref{tab:sources}). 2MASS J17112729-2725283 has a similar extinction to 2MASS J19410754+1056277 (where \choh is detected) while 2MASS J19365867+0733595 has over a magnitude less in extinction in K band than 2MASS J19410754+1056277.  However for all three sources the column densities of the polar wing of these sources are also lower by more than 30\% than the polar wings where we do detect \choh.  We calculate upper limits for the fraction of \choh:CO$_{\text{polar}}$ and find 3$\sigma$ upper limits between 0.29 and 0.72 as reported in Table \ref{tab:col density}. 

These sources without independent detections of \choh may represent an earlier stage where the hydrogenation of CO has begun and the two ices are mixed.  We expect that the YSO sources, 2MASS J17111827-2725491 and 2MASS17112729-2725283 are at high enough levels of extinction for the \choh ice to exist so perhaps the environment is affecting the ice formation.  Both are within the B59 core where turbulence from some of the YSOs has presumably prevented the core from collapsing \citep{DuarteCabral2012} so possibly this limits the CO freeze out. However the \choh:CO$_{\text{polar}}$ upper limits for both sources are not significantly lower than our detections so it is possible we merely do not have the sensitivity to detect the \choh band.   For 2MASS J19365867+0733595  the upper limit is more than 3$\sigma$ lower than our lowest \choh detection.  This source is in the background of the cloud B335 but at a lower extinction than our \choh detections so it is likely at this lower density this ice hydrogenation stage is just beginning and \choh is not overly abundant.  

It is noteworthy that all three lines of sight have high CO:H$_2$O ice ratios which could be explained if less CO ice is being consumed to make \choh ice. 

%In the earliest stage of of a molecular core ice growth depends on both the temperature and density within the core.  At low densities ($n\geq10^3$) and temperatures above 20K H$_2$O condenses onto grains mixing with other ices such as CH$_4$, CO$_2$ (polar component), and NH$_3$ (Ioppolo et al. 2011).  As temperatures decrease (T$<$20K and densities increase ($n \geq10^4$) apolar ice condenses such as CO and CO$_2$.

%In later stages the presence of a YSO can cause thermal processing causing some ices in very dense regions to start sublimating causing a segregation of molecules.  With temperatures above 90K and high energy photons we may begin to witness the formation of COMs.  ices   H$_2$O is one of the first ices to condense onto grains and mixes with others such as CH$_4$, CO$_2$, and NH$_3$ (Ioppolo et al. 2011) at relatively low densities ($n\geq10^3$) cm$^{-3}$ and warm temperatures (T$>$20K).




%and mapping their spatial distribution over a molecular core poses as a strong diagnostic tool to constrain the physical conditions required for different chemical processes to occur.  Few studies have attempted to map ices:  Murakawa et al. (2000) mapped ices in the Taurus region while Pontoppidan et al. (2004) mapped the envelope of a Class 0 YSO with background Class II LYSOs, and Pontoppidan (2006) mapped a dense core with Class I/II YSOs.  

%From the ground CO$_2$ suffers from telluric features and the CO band suffers from high sky background noise. The \choh feature 


%The discovery of exoplanets has shown that there must be a relatively common process to build up grains to form planetary bodies.  In dense molecular clouds the freeze-out of gases onto cold dust grains build up ice mantles that could lead to the growth needed to build larger bodies.  These molecules (H$_2$O, CO, CO$_2$, \choh, NH$_3$, etc.) are essential in understanding the early composition of our own solar system, however the prevalence of these molecules and the conditions promoting or inhibiting their formation (e.g., density, time scales, stellar feedback) are currently not well observationally constrained.

%While there are prolific studies of the distribution of H$_2$O, CO$_2$, and CO gas features in molecular clouds, previous studies on the ice features have mainly focused on low mass YSOs at a more evolved stage in prestellar evolution.  Very few studies have actually probed background stars of quiescent or collapsing molecular clouds for all three ices \citep{Whittet1998, Gibb2004, Noble2013}.  Some observations have studied either \hto (3.0 $\mu$m), \choh (3.53 $\mu$m), or CO (4.67 $\mu$m) ices from the ground (CO$_2$ has too much telluric absorption) but not usually simultaneously for the same stars (e.g. \cite{Whittet1985, Whittet1989, Eiroa1989, Boogert2011}).

 %so it is important to observationally constrain the pathways to develop new ice species on dust grains and study the environmental conditions that promote the ice growth.  

%When this ratio is large hydrogenation (the addition of H atoms) dominates to form molecules such as \hto, NH$_3$, and CH$_4$.  When the ratio is smaller then reactive atoms such as O and N can interact with one another forming molecules like CO, CO$_2$, O$_2$, and N$_2$ (Allamandola et al. 1999).  The H/H$_2$ ratio decreases rapidly with increased density (Hollenbach et al 1971) so when a molecular core has a relatively low density (n$>$10$^3$ cm$^{-3}$) we find \hto ice and mixtures with \hto dominate.  The ice formation threshold of A$_V$=1.6 mag near the edges of molecular cores signifies the onset of rapid ice mantle growth after an initial monolayer has been deposited.  The photodesorption decreases as the dust extinction increases allowing CH$_4$, CO$_2$, and NH$_3$ to develop as mixtures with H$_2$O.  In higher densities and lower temperatures CO accretion rates increase.  

%At the earliest stages of a molecular core when densities are relatively low (n>10^3 cm^-3) cold dry dust grain surfaces (<90K) provide a meeting point   

%As the density of molecular clouds increases and shields the core from interstellar radiation gas readily condenses onto cold dust particles (<10 K) creating icy mantles.


%Dense molecular cores provide a chemical laboratory to study interstellar ices to probe the origins of organic and volatile material of the solar nebula that perhaps formed the building blocks of life.  As the density of molecular clouds increases and shields the core from interstellar radiation the condensation of gas onto cold dust particles can occur creating icy mantles.  Chemical processes on the dust grain surfaces is key to forming new molecules in star forming regions that cannot be readily created in the gas phase \citep[and references therein]{Tielens1982, Herbst2009}.  Observationally we do not fully understand the pathways to develop new ice species on dust grains. 

%the ratio of CH$_3$OH:CO$_{\text{polar}}$=0.46 $\pm$ 0.056 for 2MASS J18172690-0438406 and 0.73 $\pm$ 0.065 for 2MASS J19410754+1056277.  The latter source traces a starless core and the ratio is higher than that of low-mass YSOs revealing that the process to form \choh abundantly from CO is possible early on.  We determine the fraction of the CO ice that has frozen out and find that much of the CO still exists in the gas phase and very little has likely been used up to make \choh ice showing that the the sampled columns are dominated by lower extinction regions. We also identify how the environment of different cores can affect ice growth.



%The cold surfaces of dust grains in dense molecular clouds are chemical factories where simple and complex organic molecules are formed. CH$_3$OH ice is a key ingredient to this process and thus it is vital to understand the onset of this ice and the conditions required for it to form.  We selected a sample of 14 stars to measure the line of sight through four small ($\sim<$2 pc in diameter) molecular clouds - both starless and with embedded young stellar objects (YSOs).  Using NASA's Infrared Telescope Facility (IRTF) SpeX instrument we simultaneously observe the H$_2$O (3.0 $\mu$m), \choh (3.53 $\mu$m) and CO (4.67 $\mu$m) features.  We model the spectral type of the stars using the IRTF spectral library of giants and calculate the baseline and find that two of our sources are embedded YSOs while the rest are background targets with A$_K$ ranging from 0.5 - 5.6 magnitudes.   We find that all of our sources have \hto ice, seven have CO ice, and two have \choh ice detections above 3$\sigma$.  We model the CO absorption feature including a polar component and find \choh/CO$_{polar}$=0.66 $\pm$ 0.09 for 2MASS J18172690-0438406 and 0.85 $\pm$ 0.85 $\pm$ 0.07 for 2MASS J19410754+1056277. This is the first measurement of this relationship for background targets and we find that it is in between the ratio for low and high mass YSOs showing that this complex molecule formation does occur before star formation. 


%The extinction maps derived by Chu et al. (in prep) using the NICEST technique \citep{Lombardi2009} use observations from UKIRT in the JHK bands and $Spitzer$ Channels 1 and 2.  An aperture with a diameter of twice the star PSF is placed at the target position and the mean extinction value inside the aperture is taken as the source's extinction value, A$_V$.  This is also reported in Table \ref{tab:sources} along with the standard deviation.  

%For each source we combined the spectra from IRTF with photometric points from 2MASS JHK and WISE Channels 1 and 2. We convolved the spectra to match the K$_S$ band from 2MASS as we do not have coverage of J and H bands in our spectra and need to ensure we calibrate the spectral fluxes to the photometry. We do not convolve the spectrum with WISE photometry since we have have full coverage of both the K band and L band spectroscopy simultaneously so calibrating to the K band is sufficient and typically has lower errors.    We then fit the calibrated spectra to the full IRTF database of observed stellar spectra \citep{Rayner2009}.  In these models we assume the extinction law from \citet{Indebetouw2005} and fit A$_K$ using a $\chi^2$ minimization routine.  Simultaneously the models fit the 3.0 $\mu$m H$_2$O ice feature  described in Section \ref{sec:water ice}.  Using the reduced $\chi^2$ values from fitting the A$_K$, the 3.0 $\mu$m ice feature, the photometric features in JHK bands, and the K band spectral features (where we detect the CO bandheads), we produce a total combined reduced $\chi^2$ value.  This reduced $\chi^2$ value provides us with the ability to sort through the IRTF models and determine the best fit and spectral type where the reduced $\chi^2$ is minimized using the method from \citet{Boogert2011}.  To determine errors on the A$_K$ we first derive the reduced $\chi^2$ from fitting the JHK photometry.  Then from the reduced $\chi^2$ distribution of all the stellar models we determine what the A$_K$ is where the reduced $\chi^2$ is 9 above the reduced $\chi^2$ of the best fit. The difference in the A$_K$ values then represents the 3 sigma error.  \textcolor{red}{The error for the spectral type is then taken to include spectral classes within a factor of 3 of the best fit reduced $\chi^2$ value.} In some cases the IRTF model does not have spectral coverage beyond the K band, since we are using these models to primarily determine the baseline for the ice features and remove photospheric lines we only consider models that extend to the L and M bands.   Parameters for the models are provided in Table \ref{tab:model_fits}.

%Some of our sources  (2MASS J18173285-0442271, J8174365-0438205, and 19365867+0733595) have high $\chi^2$ values and are best fit with late M giant templates.  The higher $\chi^2$ is due to a poor fit beyond 3.5 $\mu$m which reveals the limitations of our models in that we do not have a good representation potentially for these late type sources.  In \citet{Boogert2011} they similarly flagged later types and stated that the fitting parameters are more uncertain.

%\hangindent=0.7cm \textit{\textbf{Environment of 2MASS J18172690-0438406 (L483)}} - In Section \ref{sec:L483} we introduce the cloud L483 which has a deeply embedded (A$_V\sim70$) protostar between the Class 0 and Class I stage \citep{Tafalla2000, Fuller1995}.  2MASS J18172690-0438406 is at a lower extinction than the embedded YSO (A$_V\sim40$) and its projected distance on the sky is $\sim$14,000-18,000 AU away from the protostar in the northwest direction (similar to the distance to the Oort cloud in our own Solar System).  In Figure \ref{fig:color images} it is clear that the source is nearly orthogonal to the bipolar outflows and thus the ice growth should not be affected by the enhanced UV field or shocks from the YSO.  Preliminary extinction maps show that the background star does not appear to be sampling a different clump from the protostar as the extinction map shows a nearly spherical extinction structure around the protostar and the background star traces an outer shell (Chu et al. in prep).  Assuming turbulent fragmentation to form individual cores for low mass stars we can assume YSO envelope size scales up to the Bonnor-Ebert radius (10$^4$ AU for $n_H=10^5$ cm$^-3$, $T=$10K, \citet{Offner2010}).  This means the background star is not part of the YSO envelope and the \choh ice is forming without influence from the nearby YSO.
 
%\hangindent=0.7cm \textit{Environment of 2MASS J19410754+1056277 (L694-2)} - The shape of L694-2 as seen in Figure \ref{fig:color images} shows that a cometary tail-like shape extends to the southeast from the densest part of the starless core.  Our target 2MASS J19410754+1056277 lies within this extended feature very near the edge of the core where background sources become obscured in the K band about 0.1 pc (20,000 AU) away from the densest region.  This is evidence that even outside the highest regions of extinction \choh ices are abundant.  A similar source, 2MASS J18171181-0814012 in the starless collapsing (or near-collapsing) core L429-C also shows \choh ice outside the densest part of the core  \citep{Boogert2011, Stutz2009}.  As noted in Section \ref{sec:CO Ice Discussion} we found that the ratio of CH$_3$OH:CO$_{\text{polar}}$ for our L694-2 source is higher than the low-mass YSO L1489.


%the upper limit would decrease by $\sqrt{n}$ where $n$ is the number of spectral resolution elements in the data.  However smoothing by $n$ will reduce the peak depth of the feature and become unresolved thus we conservatively divide $N$ by $\sqrt{n/2}$ where

%\begin{equation}
%    n = FWHM \times (R \times k^{-1}).
%\end{equation}

%\noindent The wavenumber is represented as $k$ ( cm$^{-1}$) and the spectral resolution as $R$.  

%\textcolor{red}{Need to insert text about smoothing the spectra for \choh and OCN$^-$  using the boxcar method to lower our upper limits.  We used a smoothing factor of 1/2 the FWHM.}

%As seen in the correlation for the \hto feature, the cloud L483 may require higher levels of extinction for ice to form so we could be witnessing a similar effect where this source has a lower level of CO despite its high extinction.  Alternatively, we may be learning something new about CO ice at high levels of extinction.  This is the first time CO ice has been measured for a background star with an extinction above A$_K \sim 2.6$ and it may be that a linear fit is no longer applicable.  Some of the CO is perhaps lost as it is used in the formation of \choh and other more complex molecules.  Unfortunately with one source we do not have the ability to determine if there is a turnoff point where the fit is no longer linear and will require additional measurements on other targets at high extinctions.

%\begin{enumerate}
%    \item For the first time the \choh ice feature is measured simultaneously with the CO ice feature for two background targets.  The ratio of pure \choh ice to the polar wing of CO is between 0.46 and 0.73 which is similar to, yet higher than the measurement found for low-mass YSO L1489 (0.40).  This indicates that \choh formation through CO hydrogenation may be even more efficient outside of YSO envelopes than previously known.
    
%    \item CH$_3$OH ice formation is well underway before stars form. One source where CH$_3$OH was detected was in the starless core L694-2 where it is still undergoing collapse.  The distance is only about 0.1 pc ($\sim$20,000 AU) from the densest part of the core projected on the sky.  Meanwhile the second detection is slightly closer ($\sim$14,000-18,000 AU) to the core where a Class I YSO has formed.  This source probes a region outside of the YSO envelope so it has formed without necessarily direct influence from the YSO. Extinction maps of these targets will provide more insight on the structure of the cores to put these formation locations into context (Chu et al. in prep). 
    
 %   \item The ice formation threshold with respect to extinction is calculated for H$_2$O and CO. Because our sample contains cores that are at different stages of evolution we find these thresholds to vary from previous studies.  It appears that the core L483 (with a Class I YSO) requires higher levels of extinction in order for ices to form, while L694-2 (a starless collapsing core) has ices forming at lower levels of extinction.  We measure the CO ice for extinctions greater than previous studies and one source shows signs that some of the CO may be less prevalent because it is converted into other complex molecules.  However since the source is in L483, the CO is perhaps suppressed due to environmental factors.  Additional sources at high extinction levels are required to make further conclusions about the thresholds where CO is depleted due to conversion into more complex molecules.
    
  %  \item The polar wing in the CO ice absorption band is detected for three sources above 3$\sigma$ where \choh is not independently found. Two of the sources are YSOs but the ice traces the foreground cloud and not the envelopes since the YSOs are no longer envelope-dominated.  The absence of the \choh feature may be due to measuring an earlier stage of ice formation.   The hydrogenation of CO has started and the two ices are mixed but there is not enough of pure \choh for a detection at 3.53 $\mu$m.  We are possibly witnessing environmental effects where turbulence has prevented the CO freeze-out. It is unlikely that the polar wing is due to a mixture with another ice but we do note that the CO:H$_2$O ratio is rather high and could be explained if less CO ice is being consumed to make \choh ice.  we do not have the sensitivity to detect the pure \choh ice.
    
   % \item This work will be greatly improved by space-based observations with the James Webb Space Telescope (JWST) where fainter sources can be detected without high sky background noise in the 3-5 $\mu$m range.  This will improve both the ability to model the background stars more easily as well as detect ices with fainter targets.  With multiple measurements per isolate core we can develop ice maps to provide stronger conclusions for the environments and evolutionary stages in which these ices dominate.
%\end{enumerate}

==> tab-col_densities.tex <==
\begin{sidewaystable}
\tabcolsep=0.1cm
\fontsize{7}{7}\selectfont
%\tabletypesize{\tiny}
\centering
\caption{Ice Column Densities and Abundances}
\label{tab:col density}
\begin{tabular}{l|r|rr|rr|rr|rrr|rr}

\tableline\tableline
\multicolumn{13} {c} {Background Stars} \\

\tableline\tableline

\multicolumn{1}{l}{Source} & \multicolumn{1}{c}{N(H$_2$O)} & \multicolumn{2}{c}{N($_c$CO)} & \multicolumn{2}{c}{N$_r$(CO)}  & \multicolumn{2}{c}{N$_b$(CO)}  & \multicolumn{3}{c}{N(CH$_3$OH)}  & \multicolumn{2}{c}{N(OCN$^-$)} \\ 
\cmidrule(r){3-4}
\cmidrule(r){5-6}
\cmidrule(r){7-8}
\cmidrule(r){9-11}
\cmidrule(r){12-13}
2MASS J & 10$^{18}$ cm$^{-2}$ & 10$^{17}$ cm$^{-2}$ & \%\hto & 10$^{17}$ cm$^{-2}$   & \%\hto & 10$^{17}$ cm$^{-2}$   & \%\hto & 10$^{17}$ cm$^{-2}$   & \%\hto & \% CO$_r$ & 10$^{17}$ cm$^{-2}$ & \%\hto \\

% & cm$^{-2}$ &     & \%\hto & cm$^{-2}$    & \%\hto & cm$^{-2}$    & \%\hto & cm$^{-2}$    & \%\hto & \% CO$_r$\\
 \tableline
 
 17111501-2726180 & 2.46 (0.10) & $<$13.6    & $<$57.8 &    & … & …    & … &    &  & …    &  & \\
 18171765-0439379 & $<$0.55 & $<$3.1    &  & …    & … & …    & … &    &  & …    & & \\
 18172690-0438406 & 6.05 (0.11) & 5.77 (0.28) & 11.89 (0.58) & 5.18 (0.35) & 8.57 (0.60) & 1.08 (0.29) & 1.78 (0.48) & 2.37 (0.24) & 3.92 (0.41) & 45.79 (5.63) & $<$0.3 & $<$0.6 \\
 18173285-0442271 & 0.42 (0.09) & 0.58 (0.06) & 11.79 (2.17) & …    & … & …    & … & $<$1.2    & $<$29.3 & …    & $<$0.2 & $<$5.8 \\
 18174365-0438205 & 0.20 (0.03) & $<$0.8    & $<$47.0 & …    & … & …    & … &    &  & …    & & \\
 19365867+0733595 & 0.78 (0.01) & 2.65 (0.10) & 34.01 (1.55) & 1.36 (0.12) & 17.49 (1.54) & …    & … & $<$0.7    & $<$9.0 & $<$54.8    & $<$0.2 & $<$2.0 \\
 19405855+1054527 & $<$0.14 & $<$1.0    &  & …    & … & …    & … &     &  & …    &  & \\
 19410754+1056277 & 2.11 (0.07) & 6.18 (0.26) & 29.30 (3.34) & 3.87 (0.31) & 18.33 (1.62) & 0.41 (0.25) & 1.95 (1.18) & 2.80 (0.11) & 13.29 (0.70) & 72.53 (6.51) & $<$0.4 & $<$2.2  \\
 19411163+1054416 & 0.28 (0.10) & 0.49 (0.24) & 17.41 (10.59) & …    & … & …    & … &    &  & …    & & \\
\tableline\tableline                              
\multicolumn{13} {c} {Young Stellar Objects} \\
\tableline\tableline

\multicolumn{1}{l}{Source} & \multicolumn{1}{c}{N(H$_2$O)} & \multicolumn{2}{c}{N(CO)} & \multicolumn{2}{c}{N$_r$(CO)}  & \multicolumn{2}{c}{N$_b$(CO)}  & \multicolumn{3}{c}{N(CH$_3$OH)}  & \multicolumn{2}{c}{N(OCN$^-$)} \\ 
\cmidrule(r){3-4}
\cmidrule(r){5-6}
\cmidrule(r){7-8}
\cmidrule(r){9-11}
\cmidrule(r){12-13}
2MASS J & 10$^{18}$ cm$^{-2}$ & 10$^{17}$ cm$^{-2}$ & \%\hto & 10$^{17}$ cm$^{-2}$   & \%\hto & 10$^{17}$ cm$^{-2}$   & \%\hto & 10$^{17}$ cm$^{-2}$   & \%\hto & \% CO$_r$ & 10$^{17}$ cm$^{-2}$ & \%\hto \\

\tableline

 17111827-2725491 & 2.51 (0.03) & 5.30 (0.18) & 21.13 (1.03) & 2.69 (0.28) & 10.72 (1.12) & …    & … &   $<$2.7  & $<$10.9 &  $<$109.9  & $<$0.5 & $<$2.0 \\
 17112153-2727417 & 1.05 (0.04) & $<$0.8    & $<$7.4 & …    & … & …    & … & $<$1.2    & $<$12.8 & …    & $<$0.2 & $<$1.9 \\
 17112508-2724425 & 2.12 (0.04) & 1.94 (0.65) & 9.15 (3.10) & …    & … & …    & … &     &  & …    & & \\
 17112701-2723485 & 3.42 (0.06) & 1.46 (0.16) & 4.26 (0.51) & …    & … & …    & … & $<$2.4    & $<$7.3 &    & $<$0.3 & $<$1.1 \\
 17112729-2725283 & 0.46 (0.02) & 2.30 (0.13) & 50.22 (7.88) & 2.12 (0.21) & 46.38 (5.07) & 0.33 (0.12) & 7.20 (2.64) & $<$2.0    & $<$50.5 & $<$103.0    & $<$0.5 & $<$12.9 \\
\tableline\tableline


\vspace{1.cm}
\hspace{1cm}
\end{tabular}
\end{sidewaystable}

==> tab-model_fits.tex <==
\begin{table*}[h!t]
\tabcolsep=0.1cm
\tabletypesize{\small}
\centering
\caption{Continuum Fit Parameters}
\label{tab:model_fits}
\begin{tabular}{lccccc}

\tableline\tableline															
Source 	&	\multicolumn{2}{c}{IRTF\footnote{Best fitting 1-4$\mu$m spectrum from the IRTF database of \citet{Rayner2009}}}	&	A$_K$\footnote{Errors shown are 3$\sigma$}	&	$\tau_{3.0}$\footnote{Errors shown are 3$\sigma$}	&	$\chi_{\nu}^2$(total)\footnote{Averaged Reduced \chisq as described in Section \ref{sec:modeling}}	\\
ID	&	Spectral Type	&	Template	&	(Mag)	&		&		\\
\tableline											
B59-B1 	&	M6.5III	&	HD142143	&	3.59$\pm$0.17	&	1.52$\pm$0.19	&	0.54	\\
B59-Y1 	&	YSO	&	-	&	-	&	-	&	-	\\
B59-Y2 	&	YSO	&	-	&	-	&	-	&	-	\\
B59-Y3 	&	YSO	&	-	&	- 	&	-	&	-	\\
B59-Y4	&	YSO	&	-	&	-	&	-	&	-	\\
B59-Y5 	&	YSO	&	-	&	-	&	-	&	-	\\
L483-B1 	&	K4I	&	HD201065	&	0.66$\pm$0.06	&	$<$0.34	&	0.47	\\
L483-B2 	&	M6III	&	HD18191	&	4.71$\pm$0.07	&	2.79$\pm$0.15	&	2.35	\\
L483-B3	&	M7III	&	HD207076	&	0.90$\pm$0.07	&	0.22$\pm$0.14	&	9.61	\\
L483-B4	&	M7III	&	HD207076	&	0.88$\pm$0.06	&	0.12$\pm$0.05	&	18.86	\\
B335-B1 	&	M5.5III	&	HD94705	&	1.29$\pm$0.05	&	0.48$\pm$0.01	&	24.01	\\
L694-B1 	&	M5.5III	&	HD94705	&	0.51$\pm$0.06	&	0.05$\pm$0.08	&	3.59	\\
L694-B2  	&	M2III	&	HD120052	&	2.92$\pm$0.11	&	1.30$\pm$0.14	&	2.13	\\
L694-B3  	&	K3.5III	&	HD35620	&	0.74$\pm$0.06	&	0.17$\pm$0.19	&	0.46	\\
\tableline															



\vspace{0.5cm}
\end{tabular}
\end{table*}

